Enhancing Brazilian Sign Language Recognition through Skeleton Image Representation

Effective communication is paramount for the inclusion of deaf individuals in society. However, persistent communication barriers due to limited Sign Language (SL) knowledge hinder their full participation. In this context, Sign Language Recognition (SLR) systems have been developed to improve communication between signing and non-signing individuals. In particular, there is the problem of recognizing isolated signs (Isolated Sign Language Recognition, ISLR) of great relevance in the development of vision-based SL search engines, learning tools, and translation systems. This work proposes an ISLR approach where body, hands, and facial landmarks are extracted throughout time and encoded as 2-D images. These images are processed by a convolutional neural network, which maps the visual-temporal information into a sign label. Experimental results demonstrate that our method surpassed the state-of-the-art in terms of performance metrics on two widely recognized datasets in Brazilian Sign Language (LIBRAS), the primary focus of this study. In addition to being more accurate, our method is more time-efficient and easier to train due to its reliance on a simpler network architecture and solely RGB data as input.

==> secs/backup/2-method-backup.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/overview.pdf}
  \caption{Overview of the proposed ISLR method. Initially, landmarks are extracted from individual frames of the input video sequence. Then, the landmarks are converted into a single 2-D image that encodes spatial and temporal information. Finally, the image is fed into a CNN model for sign classification.}
  \Description{The image illustrates a process for sign language recognition. It begins with "Input frames" showing a man performing a sign with his hands. Next, "Landmarks extraction" highlights his face and hands with red, blue, and green marks to identify key points. Following is "Image encoding," which displays an abstract representation of these landmarks. This is then fed into a "CNN", resulting in an "Inference" where the sign is recognized as "to happen". The process flow is depicted with arrows between each step.}
  \label{fig:overview}
\end{figure}

\section{Proposed ISLR Method}
\label{sec:method}

% Figure \ref{fig:train_flowchart} outlines the training process, tracing the workflow from the initial raw dataset to the model evaluation. The diagram is segmented into three critical phases: data preparation, data augmentation, and image transformation. This section will detail these steps.

The basic pipeline of the proposed method is illustrated in Figure \ref{fig:overview}. Initially, the frames of the input video sequence, comprising a single sign, are processed individually to extract body, hands, and face landmarks. Each landmark point consists of three components: the 2-D spatial coordinates and the time position, corresponding to the frame from which it was extracted. Subsequently, the landmarks are converted into a single 2-D image that encodes both spatial and temporal information. This image is then fed into a CNN model, which outputs the class label of the sign with maximum probability (sign label). The following sections describe each part of the presented pipeline, as well as the process to train the CNN model.

\subsection{Landmarks Extraction}
\label{sec:landmarks-extraction}
% In sign language, a word is represented by a sign, which involves specific hand shapes, movements, and locations. Additionally, some signs incorporate facial expressions and non-manual markers such as eyebrow movements, head tilts, or eye gaze, which can convey questions, negation, emphasis, or other linguistic elements. In the literature on Sign Language Recognition (SLR), two prevalent approaches are RGB-D and Landmarks. The RGB-D approach utilizes videos enhanced with depth data captured by Kinect or Leap Motion sensors, effectively employing 3D CNN networks that process multiple images as input. The Landmarks approach focuses on extracting data from key body points along the X, Y and Z axes, facilitating the use of Recurrent Neural Networks, such as LSTMs, for analysis.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/five_sign.png}
%   \caption{The sign for the word ``Five'' in Libras}
%   \Description{Adicionar}
%   \label{fig:five_sign}
% \end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/mirror_sign.png}
%   \caption{The sign for the word ``Mirror'' in Libras}
%   \Description{Adicionar}
%   \label{fig:mirror_sign}
% \end{figure}

% Figure \ref{fig:five_sign} displays the sign for ``Five'' in Libras, which can be categorized as "simple" due to its composition of a single static gesture. Yet, Figure \ref{fig:mirror_sign} illustrates the sign for ``Mirror'', which involves rotating the hand to perform the sign correctly, can be a little more "challenge" to categorize.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/landmarks.pdf}
  \caption{Extraction of landmarks from raw RGB frames using OpenPose \cite{cao2019openpose}. All landmarks above the hip (totaling 126) were utilized, including 42 hand landmarks (green dots), 70 face landmarks (yellow dots), and 14 body landmarks (red `x'). Face points indicated by `x' markers are treated as body landmarks by OpenPose.}
  \Description{The image shows a man against a green background performing a sign with his hands. Overlaid on the image are various colored dots and crosses, marking key points on his face (yellow dots), hands (green dots), and body (red crosses). A close-up inset of the man's face with the same landmarks is provided on the right for detail.}
  \label{fig:landmarks}
\end{figure}

In this initial stage, the space-time landmarks are extracted from the raw RGB frames of the input video sequence. This extraction process relies on OpenPose \cite{cao2019openpose}, a deep learning-based open-source library for estimating human poses by extracting 2-D keypoints. OpenPose has been widely used in various applications, including movement analysis in sports \cite{chen2023research} and physiotherapy \cite{saiki2023reliability}, as well as human activity recognition \cite{emanuel2021snapshot}. Due to its capability to detect facial features, which are crucial for Sign Language Recognition (SLR), OpenPose is also utilized to incorporate facial elements into machine learning models for SLR \cite{DeCastro2023}.

To capture movement and facial features, all landmarks above the hip were utilized, which corresponds to 126 landmarks from a total of 137 provided by OpenPose. As depicted in Figure \ref{fig:landmarks}, there are 42 points representing the landmarks of both hands, denoted by the green dots, 70 yellow points correspond to face landmarks, and 14 red `x' markers indicating body landmarks (the 5 points situated in the face are treated as body landmarks by OpenPose). Finally, the depth coordinate inferred by OpenPose was discarded since our method focuses on 2-D data.

% The data preparation phase is designed to transform these videos into a structured landmark dataset. This involves extracting landmarks from every frame of each video and systematically organizing them into a Pandas DataFrame.  Figure \ref{fig:landmarks_extraction} demonstrates the process of landmark extraction. It displays the raw image, a composite image blending the raw image with the extracted landmarks, and finally, an image showing only the extracted landmarks.

% The final stage of data preparation involves the selective removal of unnecessary landmarks. While OpenPose generates landmarks across the X, Y, and Z axes, all Z-axis values are omitted in this process. Additionally, landmarks located below the hips are also discarded, reflecting the emphasis on hand and face movements in sign language gestures.

% One tested step was to make sure all videos from the same dataset had the same amount of frames. Besides not present on the final pipeline, it showed important results and it's explored by the ablation study in Section \ref{sec:ablation_study}. The initial step involves analyzing the distribution of frame counts across the videos, given the presence of both shorter and longer videos within the dataset. The purpose of this analysis is to identify an optimal number of frames that minimizes the removal of frames from longer videos while also avoiding excessive repetition of the same frame in shorter videos. For each video, the following steps are implemented:

% \begin{enumerate}
% \item If the video already contains the target number of frames, no action is required;
% \item If the video has fewer frames than the target, the final frame is replicated until the video meets the desired frame count;
% \item If the video exceeds the target number of frames, excess frames are removed at equally spaced intervals to achieve the desired total.
% \end{enumerate}

\subsection{Image Encoding}
\label{sec:image_transformation}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.3\linewidth]{figs/08BanheiroSinalizador01-2.mp4.png}
%   \caption{The sign for the word ``Bathroom'' represented as image by our image transformation pipeline}
%   \Description{Adicionar}
%   \label{fig:bathroom_image_repr}
% \end{figure}

% One tested step was to make sure all videos from the same dataset had the same amount of frames. Besides not present on the final pipeline, it showed important results and it's explored by the ablation study in Section \ref{sec:ablation_study}. The initial step involves analyzing the distribution of frame counts across the videos, given the presence of both shorter and longer videos within the dataset. The purpose of this analysis is to identify an optimal number of frames that minimizes the removal of frames from longer videos while also avoiding excessive repetition of the same frame in shorter videos. For each video, the following steps are implemented:

% \begin{enumerate}
% \item If the video already contains the target number of frames, no action is required;
% \item If the video has fewer frames than the target, the final frame is replicated until the video meets the desired frame count;
% \item If the video exceeds the target number of frames, excess frames are removed at equally spaced intervals to achieve the desired total.
% \end{enumerate}

The image encoding is achieved through the Skeleton-DML algorithm \cite{memmesheimer2022skeleton}. Although originally intended for representing skeleton joints for human activity recognition, the underlying concept applies to space-time coordinates in general, as is the case with the landmarks in our method. Additionally, adapting to 2-D coordinates is straightforward, as omitting the depth coordinate (z-axis) simply implies waiving a portion of the image data. The following paragraph describes more formally the encoding process.

Given a video sequence with $T$ frames, the set of extracted landmarks for a frame $j \in \{1, 2, \ldots, T\}$ can be represented as coordinates $\{(x^{(j)}_i,~y^{(j)}_i)\}_{i=1}^{L}$, where $L=126$ is the total number of landmarks. The $x$ and $y$ coordinates are real values normalized into the $[0,1]$ range. In the encoding process, the coordinates are converted into the matrices $\mathbf{X}=[X_{ij}]_{L \times T}$ and $\mathbf{Y}=[Y_{ij}]_{L \times T}$, where $X_{ij} = x^{(j)}_i$ and $Y_{ij} = y^{(t)}_i$. The matrices are reshaped into $L \times T / 3 \times 3$ tensors $\mathbf{X}'$ and $\mathbf{Y}'$, so that $X'_{ijk} = X_{i,3j+k}$ and $Y'_{ijk} = Y_{i,\,3j+k}$.
% Since $T$ \px{is a multiple of 3}, the number of columns, $T/3$, is integer.
Finally, the encoded image corresponds to $I = \mathbf{X}' \oplus \mathbf{Y}'$, where $\oplus$ denotes the concatenation along the horizontal axis. The values of $I$ are scaled to integer values in the $[0, 255]$ range. Notice that $I$ is a 3-channel (RGB) image with $L$ rows and $2T/3$ columns.

It is worth mentioning that the interpretation of the generated image is not straightforward. As shown in Figure \ref{fig:overview}, dark and bright pixels indicate the leftmost and rightmost positions in the frame, respectively. Furthermore, constant rows indicate that the position of the associated landmark is not changing considerably. Colored pixels, on the other hand, represent fast movements, indicating sharp variations in the horizontal and/or vertical direction within a 3-length temporal window.

% For each video, landmarks are extracted and subsequently transformed into a single image. This process involves capturing the landmarks from the X and Y axes and converting them into two arrays. These arrays are then reshaped from two dimensions into three dimensions, specifically: the number of columns, the number of rows, and the number of channels. Three channels are used, corresponding to the red, green, and blue colors. The number of rows is represented by -1 value, instructing to automatically calculate the dimension that best fits the transformation while the number of columns is represented by the same number of columns of the original array.

% Figure \ref{fig:bathroom_image_repr} illustrates the result of the image transformation process for the ``Bathroom'' sign. Although the transformed image may not be interpretable by humans, the model is designed to understand and accurately categorize the sign language gesture.

\subsection{Training the Model}
\label{sec:model}

The training of the model leverages a collection of annotated videos, each one comprising a single sign. In a preliminary (offline) step, each video sequence is processed to extract and store the respective landmarks. In each training epoch, the landmarks undergo an augmentation procedure before being converted into 2-D images to train the convolutional model. The augmentation process aims to enhance data diversity across training epochs by applying basic transformations, including rotation, zoom, translation, and horizontal flip. In our approach, this process does not increase the number of samples.


% \subsubsection{Data Augmentation}
% \label{sec:data_augmentation}

% Data augmentation is executed on-the-fly directly on the landmarks using a custom PyTorch Dataset. This dataset ingests a DataFrame that encapsulates the landmarks from each video and is responsible for producing an image, a process that will be elaborated upon in the Image transformation subsection. Before converting the landmarks into an image, several augmentation techniques are applied to the landmarks: rotation, zoom, translation, and horizontal flip. The parameters for rotation, zoom, and translation on X axis are selected based on a random normal distribution, with each factor having its own predefined standard deviation. The horizontal flip value determines it's probability. The defined parameters are: 0.12 for rotation, 0.1 for zoom, 0.06 for translation and 0.3 for mirroring.

The adopted CNN architecture consists of an 18-layer Deep Residual Network (ResNet18) \cite{he2016deep} (base network), followed by two fully connected layers: a 128-unit layer with ReLU activation for feature extraction, and an output layer whose size matches the number of signs (classes) in the dataset. The input size of the network is $224 \times 224$, while the encoded images have dimensions $126 \times 2T/3$. Although the length of the video sequences $T$ may vary across the samples, the encoded image width ($2T/3$) is consistently lower than 224 for the evaluated cases. Indeed, having $L \geq 224$ would imply shot lengths of approximately 11 seconds (assuming a frame rate of 30 fps), which is unlikely for isolated signs. Therefore, there is no loss of information when resizing the image to fit the network input size because the image dimensions are always increased.

During training, the base network is initialized with pre-trained weights from ImageNet. The model undergoes training for 20 epochs using the Adam algorithm to minimize cross-entropy loss, with a mini-batch size of 64, and a learning rate of 0.0001. An early stopping mechanism is implemented, halting training if the validation loss fails to decrease over five consecutive epochs. To mitigate overfitting, batch normalization is applied to the output of the base network, and dropout regularization with a probability of 0.5 is employed after the 128-unit layer. Furthermore, L2-regularization with a weight of 0.0001 is applied to the network parameters. The model state of the epoch that achieved the highest validation accuracy was chosen as the ``best model'' for posterior evaluation.

% The developed model employs a ResNet18 architecture with pre-trained ImageNet weights, where the Fully Connected layer has been substituted with a sequence of layers aimed at enhancing performance and reducing overfitting. This sequence includes a Batch Normalization layer, followed by a Dense layer with 128 units and ReLU activation, a Dropout layer with a rate of 0.5 and another Dense layer designed to correspond with the number of signs in the dataset. Optimization is handled by an Adam Optimizer with a learning rate and weight decay both set at 0.0001. The model was trained for 20 epochs, with a Cross Entropy loss, a mini-batch size of 64 and incorporating an early stopping mechanism that halted training if the validation loss failed to decrease over five consecutive epochs. The epoch that achieved the highest validation accuracy was subsequently chosen as the "best model."

% %%%
% As noted in the introduction, the ``\verb|acmart|'' document class can
% be used to prepare many different kinds of documentation --- a
% dual-anonymous initial submission of a full-length technical paper, a
% two-page SIGGRAPH Emerging Technologies abstract, a ``camera-ready''
% journal article, a SIGCHI Extended Abstract, and more --- all by
% selecting the appropriate {\itshape template style} and {\itshape
%   template parameters}.

% This document will explain the major features of the document
% class. For further information, the {\itshape \LaTeX\ User's Guide} is
% available from
% \url{https://www.acm.org/publications/proceedings-template}.

% \subsection{Template Styles}

% The primary parameter given to the ``\verb|acmart|'' document class is
% the {\itshape template style} which corresponds to the kind of publication
% or SIG publishing the work. This parameter is enclosed in square
% brackets and is a part of the {\verb|documentclass|} command:
% \begin{verbatim}
%   \documentclass[STYLE]{acmart}
% \end{verbatim}

% Journals use one of three template styles. All but three ACM journals
% use the {\verb|acmsmall|} template style:
% \begin{itemize}
% \item {\verb|acmsmall|}: The default journal template style.
% \item {\verb|acmlarge|}: Used by JOCCH and TAP.
% \item {\verb|acmtog|}: Used by TOG.
% \end{itemize}

% The majority of conference proceedings documentation will use the {\verb|acmconf|} template style.
% \begin{itemize}
% \item {\verb|acmconf|}: The default proceedings template style.
% \item{\verb|sigchi|}: Used for SIGCHI conference articles.
% \item{\verb|sigchi-a|}: Used for SIGCHI ``Extended Abstract'' articles.
% \item{\verb|sigplan|}: Used for SIGPLAN conference articles.
% \end{itemize}

% \subsection{Template Parameters}

% In addition to specifying the {\itshape template style} to be used in
% formatting your work, there are a number of {\itshape template parameters}
% which modify some part of the applied template style. A complete list
% of these parameters can be found in the {\itshape \LaTeX\ User's Guide.}

% Frequently-used parameters, or combinations of parameters, include:
% \begin{itemize}
% \item {\verb|anonymous,review|}: Suitable for a ``dual-anonymous''
%   conference submission. Anonymizes the work and includes line
%   numbers. Use with the \verb|\acmSubmissionID| command to print the
%   submission's unique ID on each page of the work.
% \item{\verb|authorversion|}: Produces a version of the work suitable
%   for posting by the author.
% \item{\verb|screen|}: Produces colored hyperlinks.
% \end{itemize}

% This document uses the following string as the first command in the
% source file:
% \begin{verbatim}
% \documentclass[sigconf,authordraft]{acmart}
% \end{verbatim}



% \subsection{Math Equations}
% You may want to display math equations in three distinct styles:
% inline, numbered or non-numbered display.  Each of the three are
% discussed in the next sections.

% \subsection{Inline (In-text) Equations}
% A formula that appears in the running text is called an inline or
% in-text formula.  It is produced by the \textbf{math} environment,
% which can be invoked with the usual
% \texttt{{\char'134}begin\,\ldots{\char'134}end} construction or with
% the short form \texttt{\$\,\ldots\$}. You can use any of the symbols
% and structures, from $\alpha$ to $\omega$, available in
% \LaTeX~\cite{Lamport:LaTeX}; this section will simply show a few
% examples of in-text equations in context. Notice how this equation:
% \begin{math}
%   \lim_{n\rightarrow \infty}x=0
% \end{math},
% set here in in-line math style, looks slightly different when
% set in display style.  (See next section).

% \subsection{Display Equations}
% A numbered display equation---one set off by vertical space from the
% text and centered horizontally---is produced by the \textbf{equation}
% environment. An unnumbered display equation is produced by the
% \textbf{displaymath} environment.

% Again, in either environment, you can use any of the symbols and
% structures available in \LaTeX\@; this section will just give a couple
% of examples of display equations in context.  First, consider the
% equation, shown as an inline equation above:
% \begin{equation}
%   \lim_{n\rightarrow \infty}x=0
% \end{equation}
% Notice how it is formatted somewhat differently in
% the \textbf{displaymath}
% environment.  Now, we'll enter an unnumbered equation:
% \begin{displaymath}
%   \sum_{i=0}^{\infty} x + 1
% \end{displaymath}
% and follow it with another numbered equation:
% \begin{equation}
%   \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
% \end{equation}
% just to demonstrate \LaTeX's able handling of numbering.

% \subsection{Figures}

% The ``\verb|figure|'' environment should be used for figures. One or
% more images can be placed within a figure. If your figure contains
% third-party material, you must clearly identify it as such, as shown
% in the example below.
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{sample-franklin}
%   \caption{1907 Franklin Model D roadster. Photograph by Harris \&
%     Ewing, Inc. [Public domain], via Wikimedia
%     Commons. (\url{https://goo.gl/VLCRBB}).}
%   \Description{A woman and a girl in white dresses sit in an open car.}
% \end{figure}

% Your figures should contain a caption which describes the figure to
% the reader.

% Figure captions are placed {\itshape below} the figure.

% Every figure should also have a figure description unless it is purely
% decorative. These descriptions convey what’s in the image to someone
% who cannot see it. They are also used by search engine crawlers for
% indexing images, and when images cannot be loaded.

% A figure description must be unformatted plain text less than 2000
% characters long (including spaces).  {\bfseries Figure descriptions
%   should not repeat the figure caption – their purpose is to capture
%   important information that is not already provided in the caption or
%   the main text of the paper.} For figures that convey important and
% complex new information, a short text description may not be
% adequate. More complex alternative descriptions can be placed in an
% appendix and referenced in a short figure description. For example,
% provide a data table capturing the information in a bar chart, or a
% structured list representing a graph.  For additional information
% regarding how best to write figure descriptions and why doing this is
% so important, please see
% \url{https://www.acm.org/publications/taps/describing-figures/}.

==> secs/backup/3-experiments-backup.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figs/sign_count_hist.png}
  \caption{Distribution of video sequence length per sign for the evaluation datasets.}%  
  \Description{The image displays two bar charts with the titles "Category count for MINDS-Libras dataset" and "Category count for LIBRAS-UFOP dataset." The left chart has uniform bars around the count of 60 for various signs labeled in Portuguese. The right chart shows varying bar heights for signs labeled by numbers, indicating a range of counts from about 40 to 60. Both charts use a blue color scheme for the bars.}
  \label{fig:sig_count_hist}
\end{figure}

\section{Experimental Methodology}
\label{sec:experiments}

This section provides a comprehensive overview of the methodology employed in this investigation, covering the selection and preparation of public datasets, the choice of performance metrics for model evaluation, and the details of the experimental procedure.

\subsection{Datasets}
\label{sec:datasets}

The datasets utilized in our experiments comprise video sequences depicting isolated signs in Brazilian Sign Language (LIBRAS). We leveraged two prominent public collections for this purpose: the MINDS-Libras dataset \cite{Rezende2021} and the LIBRAS-UFOP dataset \cite{Cerna2021}. Our literature review indicates that these datasets play a central role in ISLR in LIBRAS, enabling us to compare our method to the literature. Figure \ref{fig:sig_count_hist} shows the distribution of video sequence length per sign for both datasets. The charts demonstrate that both collections are reasonably balanced, ensuring that the number of data points for each class is approximately equal.

\paragraph{MINDS-Libras Dataset} This collection includes a subset of 20 distinct signs in LIBRAS selected by a specialist. The signs were selected by their phonological characteristics, which include aspects like hand configuration, location and movements, palm orientation, and facial expressions. They were performed by 12 signers, each signer executed the same sign five times resulting in a total of 1,158 video sequences. This number falls slightly short of the expected 1,200 samples due to the absence of certain signs from four signers. The performed signs (classes) include: ``To happen'', ``Student'', ``Yellow'', ``America'', ``To enjoy'', ``Candy'', ``Bank'', ``Bathroom'', ``Noise'', ``Five'', ``To know'', ``Mirror'', ``Corner'', ``Son'', ``Apple'', ``Fear'', ``Bad'', ``Frog'', "Vaccine'', and ``Will''.

\paragraph{LIBRAS-UFOP Dataset} This collection encompasses a subset of 56 distinct signs in LIBRAS performed by 5 signers. As detailed in \cite{DeCastro2023}, the signs are classified into four categories based on the similarity level of movement, articulation point, hand pose, and facial expression (a sign may belong to more than one category): (i) same movement and articulation point but different hand pose; (ii) different movements but the same articulation point and hand configuration (19 signs); (iii) same movement and hand configuration but different articulation points (8 signs); (iv) similar movement but different facial expression (19 signs). The similarity between signs presents a challenging factor in this dataset.
% These signs are categorized into four groups, with a sign potentially belonging to more than one category: (i) 10 signs exhibit the same movement and articulation point but different hand configurations; (ii) 19 signs demonstrate different movements but the same articulation point and hand configuration; (iii) 8 signs involve the same movement and hand configuration but different articulation points; (iv) and finally, 19 signs incorporate facial expressions and similar movements.
In contrast to MINDS-Libras, each video recording contains from 8 to 16 takes of the same sign performed sequentially. To accurately segment the time frame of each sign sample, we used an auxiliary labeling file provided along the dataset. This file specifies the precise frame where each sign begins and ends for every repetition across all videos, ensuring precise delineation of sign boundaries. Unlike MINDS-Libras, the time window of a sign in LIBRAS-UFOP does not encompass frames in which the signer is at rest position. To ensure consistency between both datasets, we included the 15 frames preceding and following the annotated frames.

\subsection{Performance Metrics}

The performance analysis leveraged four commonly used metrics in the SLR literature: accuracy, precision, recall, and F1-score. Accuracy measures the overall correctness of the model as the ratio of correct predictions to total predictions. Precision assesses the accuracy of positive predictions, calculated as the ratio of true positives to all positive predictions. Recall, or sensitivity, quantifies the model's ability to identify all relevant instances, calculated as the ratio of true positives to actual positives. The classes are weighted equally in the metrics computation, therefore, we reported the macro average of precision and recall. F1-score harmonizes precision and recall into a single metric, useful for comparing models with similar accuracies but different precision and recall values.

\subsection{Experimental Procedure}
\label{sec:exp-procedure}

% Data preprocessing
The basic experimental procedure to evaluate the efficacy of the proposed method is described as follows. In a preliminary stage, the body, hand, and face landmarks were extracted from the raw video sequences, as described in Section \ref{sec:landmarks-extraction}. We assume that, at this point, the signs in the LIBRAS-UFOP dataset were already individualized according to the procedure described in Section \ref{sec:datasets}. The following steps are applied for each dataset individually.

The partitioning of train-test samples adheres to a nested \emph{Leave One Person Out} (LOPO) cross-validation protocol, reflecting real-world application scenarios where the recognition system must operate without prior knowledge of the current signer. Following this approach, the train partition was further subdivided into exclusive train and validation sets, with each of the remaining signers used once to compose the validation set. This set was used to determine the best model, as discussed in Section \ref{sec:model}. Consequently, for a dataset comprising $n$ signers, a total of $n(n-1)$ train-test sections were conducted, ensuring thorough evaluation and robustness of the recognition system across diverse signer profiles.

In each training epoch of an experiment (section), the landmarks designated exclusively for training underwent the augmentation procedure before being converted into images, as detailed in Section \ref{sec:model}. Conversely, validation and test landmarks in each experiment were only converted into images once. Following the training phase, the model was evaluated on the corresponding test set, and the performance metrics were recorded.

\paragraph{Ablation Study} This study aims to assess the impact of excluding data augmentation from the training stage process, along with the potential benefits of implementing a mechanism to uniformize the number of frames per video sequence. The uniformization mechanism, adapted from \cite{da2024multiple}, involves setting a target number of frames per dataset and adjusting the frame count of each video sequence accordingly. Specifically, if a video contains fewer frames than the target, its last frame is duplicated until the desired count is reached. Conversely, if a video exceeds the target, frames are removed at spaced intervals to achieve the desired total, ensuring consistency across the dataset. The target frame count is determined as the average number of frames across the dataset. This study follows the outlined experimental procedure, with the difference that each investigated component is individually enabled or disabled (one-at-a-time approach). The resulting outcomes are then compared to the proposed method configuration, where augmentation is enabled and no uniformization mechanism is implemented.

\paragraph{Comparative Evaluation} The proposed method was compared to the state-of-the-art multi-stream 3D CNN architecture developed by De Castro et al. \cite{DeCastro2023}. This model integrates segmented hands and faces, pose information, speed maps, RGB images, and artificially generated depth maps. It achieved superior accuracy compared to the machine learning models developed by Passos et al. \cite{Passos2021} on MINDS-Libras and LIBRAS-UFOPS, and outperformed the multimodal approach of Cerna et al. \cite{Cerna2021} on LIBRAS-UFOP.

\subsection{Experimental Platform}

The experimental platform utilized Ubuntu 18.04.5 operating through Windows Subsystem for Linux (WSL) on a Windows 11 platform. The hardware configuration included an Intel i7 13700K processor clocked at 5.4GHz, 32GB of DDR4 RAM operating at 3200MT/s, and an NVidia RTX 4070 GPU. The development of the proposed neural network was carried out using Python v3.9.16, PyTorch 2.0.1, and CuDNN version 11.8.
The source code and pre-trained models will be publicly available upon acceptance of this work.


==> secs/backup/4-results-backup.tex <==
% https://www.evidentlyai.com/classification-metrics/multi-class-metrics
% Precision and recall metrics are also not limited to binary classification. You can use them in multi-class classification problems as well. 

% However, there are different approaches to how to do that, each with its pros and cons. 

% In the first case, you can calculate the precision and recall for each class individually. This way, you get multiple metrics based on the number of classes you have in the dataset.
% In the second case, you can "average" precision and recall across all the classes to get a single number. You can use different methods to average the precision, such as macro- or micro-averaging.
\section{Results and Discussion}
\label{sec:results}

% This section details the results achieved by our model, as defined in Section \ref{sec:experiments}, segmented by each dataset. It also discusses these results in comparison to state-of-the-art models.

Table \ref{tab:default} shows the results obtained with the proposed method in the default configuration. For the MINDS-Libras dataset, the proposed method achieved an accuracy of 0.93, precision of 0.94, recall of 0.93, and F1-score of 0.93. For LIBRAS-UFOP, accuracy was 0.82, with a precision of 0.83, recall of 0.81, and F1-score of 0.82. The remarkable difference in performance is consistent with findings in the literature \cite{DeCastro2023,Passos2021}, highlighting LIBRAS-UFOP as a more challenging dataset.
% \stboldt{Não entendi porque 0.92 e 0.82 são similares!}
% \dudu{Pois é, achei melhor remover. Precisamos de uma frase para fechar a introdução da sessão ou podemos deixar só os resultados?} \boldt{Não consegui pensar em nada.} 

\begin{table}[t]
    \centering
    \caption{Results of the proposed method in its default configuration (avg. metric $\pm$ standard deviation).}
    \Description{Teste}
    \begin{tabular}{ccccc}
        \toprule
        Dataset      & Accuracy        & Precision       & Recall          & F1-score        \\
        \midrule
        MINDS-Libras & 0.93 $\pm$ 0.05 & 0.94 $\pm$ 0.05 & 0.93 $\pm$ 0.05 & 0.93 $\pm$ 0.05 \\
        LIBRAS-UFOP  & 0.82 $\pm$ 0.04 & 0.83 $\pm$ 0.05 & 0.81 $\pm$ 0.05 & 0.80 $\pm$ 0.05 \\
        \bottomrule
    \end{tabular}
    \label{tab:default}
\end{table}

% \subsection{MINDS-Libras results}

The confusion matrix in Figure \ref{fig:confusion_matrix_minds}, normalized by true values (row values), offers an in-depth analysis of the recognition performance within the MINDS-Libras Dataset. The y-axis denotes the true label for each sign, while the x-axis reflects the labels predicted by our model. The main diagonal represents the precision for each sign. Out of 20 signs, 15 achieved a precision of at least 0.9, whereas only one sign, ``Fear'', registered a precision of 0.85. This sign was frequently misidentified as ``Son'',  ``Bad'', or ``Student''. The best performance was observed for ``America'', with a precision of 1.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.7\linewidth]{figs/confusion_matrix_minds.png}
  \caption{Confusion matrix for the MINDS-Libras dataset.}
  \Description{The image shows a confusion matrix for the MINDS-Libras dataset, which is a tool used to evaluate the performance of a classification model. The matrix is a square grid with both the columns and rows labeled with English translations of sign language categories such as ``To happen'', ``Student'', ``Yellow'', and ``America'', among others. The cells within the matrix represent the proportion of predictions, with diagonal cells from top left to bottom right showing high values (e.g., 0.94 for ``To happen'', 0.95 for ``Candy'', 0.99 for ``Mirror''), indicating correct classifications. These values are color-coded with shades of blue, with darker shades representing higher values. Off-diagonal cells mostly contain zeros or very low values, representing few misclassifications. The color bar on the right indicates the scale from 0 to 1. The overall diagonal trend suggests that the model has a high accuracy in predicting these categories.}
  \label{fig:confusion_matrix_minds}
\end{figure}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.7\linewidth]{figs/accuracy_by_signaler_minds.png}
%   \caption{Accuracy for each signaler in test and validate dataset for MINDS-Libras.}
%   \Description{A square heatmap plot displaying the average accuracy for each signaler in test and validate dataset.}
%   \label{fig:accuracy_by_signaler_minds}
% \end{figure}

% The MINDS-Libras dataset comprises 20 signs executed by 12 signalers. Using the LOPO protocol for each signaler, we conducted a comprehensive training and evaluation of the neural network, ensuring that we separate a single signaler only for the test dataset. This methodological approach is designed to validate the robustness and accuracy of our proposed method, emphasizing its capacity to recognize the signs themselves rather than adapting to the unique characteristics of the signalers in the train dataset. By adopting this strategy, we aim to highlight the efficacy of our architecture in distinguishing between the intended signs across a diverse set of signalers.

% Table \ref{tab:results} presents the performance metrics of our proposed method on the MINDS-Libras dataset, where it achieved an accuracy of 0.87, along with a precision of 0.97, recall of 0.86, and an F1-Score of 0.86.

% Figure \ref{fig:confusion_matrix_minds} illustrates a confusion matrix for the dataset's signs.  Correct predictions are indicated along the principal diagonal, whereas off-diagonal elements represent the misclassification percentage for each label.

% The analysis of the confusion matrix reveals that our model achieved an accuracy of at least 0.9 for 10 out of the 20 signs and at least 0.81 in 19 out of the 20 signs. Notably, the sign for "fear" recorded an accuracy of 0.63, the lowest among the dataset. It was frequently misidentified as "Bag", "Vaccine", or "Will", indicating areas where our model's differentiation between similar signs could be improved.

% Figure \ref{fig:accuracy_by_signaler_minds} illustrates the average accuracy obtained across various combinations of validation and test datasets. The x-axis represents the signaler designated to the validation dataset, while the y-axis corresponds to the signaler included in the test dataset. Displayed values indicate the average accuracy observed per fold. Notably, the principal diagonal is marked with a value of -1, meaning that a signaler cannot be simultaneously allocated to both datasets.
% This visualization confirms the robustness of our proposed architecture, which achieves an accuracy of at least 0.9 in 75\% of cases across diverse combinations of signalers in the validation and test datasets. Such findings suggest that our model exhibits strong generalization capabilities in classifying sign language gestures. Additionally, it is observed that the model's performance dips when signaler 4 is part of the test dataset, indicating areas for potential model improvement in future iterations.

% \subsection{LIBRAS-UFOP results}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{figs/confusion_matrix_ufop.png}
%   \caption{Confusion Matrix for LIBRAS-UFOP results achieved with our method.}
%   \Description{A Confusion Matrix plot showing the prediction percentage between all categories for LIBRAS-UFOP Dataset}
%   \label{fig:confusion_matrix_ufop}
% \end{figure}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.7\linewidth]{figs/accuracy_by_signaler_ufop.png}
%   \caption{Accuracy for each signaler in test and validate dataset for LIBRAS-UFOP.}
%   \Description{A square heatmap plot displaying the average accuracy for each signaler in test and validate dataset.}
%   \label{fig:accuracy_by_signaler_ufop}
% \end{figure}


% The LIBRAS-UFOP dataset comprises 56 signs executed by 10 signalers. In alignment with our approach for the MINDS-Libras dataset, we applied the Leave One Person Out (LOPO) protocol to each signaler for this dataset as well.

% Table \ref{tab:results} details the performance metrics of our proposed method on the LIBRAS-UFOP dataset, where it achieved an accuracy of 0.84. This represents the highest accuracy metric in comparison to other state-of-the-art methodologies, also present in the table. Furthermore, the model demonstrated a precision of 0.88, a recall of 0.84, and an F1-Score of 0.82.

% TO INCLUDE (Libras Ufop)
% An analysis of the confusion matrix, available on the supplementary material, reveals that 25 out of the 56 signs achieved an accuracy of at least 0.9, while 36 signs recorded an accuracy rate of at least 0.8. However, five signs ``Year 1'', ``Year 3'', ``Day 1'', ``Day 3'', and ``Hen'' registered precision below 0.5. On a positive note, five other signs ``Yesterday'', ``Bodybuilding'', ``Always'', ``Strong Wind'', and ``Thin'' achieved a precision of 1, being able to predict correctly 100\% of the test samples.

% The sign ``Hen'', part of category 3 which includes signs that share the same movement and hand configuration but differ in articulation point, was often mispredicted as ``Exchange'', another sign from the same category. The other signs with low precision are in category 1, characterized by the same movement and articulation point but different hand configurations. These were also often confused with signs within their category. These results indicate that while the model is capable of accurately predicting signs that are similar, there is still room for improvement in distinguishing subtle differences.


% Figure \ref{fig:accuracy_by_signaler_ufop} provides an overview of the average accuracy achieved across each fold of the dataset. It demonstrates that, across all folds, the model consistently achieved a stable level of accuracy, regardless of which signaler was allocated to the test dataset. This consistency underscores the robustness of our network architecture, illustrating its capability to accurately learn the distinctive characteristics of sign language gestures and, subsequently, to correctly predict the signs performed by signalers who were not included in the training dataset.

\begin{table}[t]
    \centering
    \caption{Results of the ablation study (avg. metric $\pm$ standard deviation). The second and third columns specify the enabled features. The first row for each dataset represents the method in its default configuration.}
    \begin{tabular}{ccccccc}
        \bottomrule
        Dataset & Data aug. & Uniform. & Accuracy & Precision  & Recall & F1-score \\
        \midrule
        \multirow{3}{*}{MINDS-Libras} & \checkmark & & 0.93 $\pm$ 0.05 & 0.94 $\pm$ 0.05 & 0.93 $\pm$ 0.05 & 0.93 $\pm$ 0.05 \\
                                      & \checkmark & \checkmark & 0.88 $\pm$ 0.08 & 0.89 $\pm$ 0.06 & 0.87 $\pm$ 0.08 & 0.86 $\pm$ 0.09 \\
                                      & & & 0.92 $\pm$ 0.06 & 0.93 $\pm$ 0.06 & 0.92 $\pm$ 0.06 & 0.91 $\pm$ 0.07 \\
        \midrule
        \multirow{3}{*}{LIBRAS-UFOP} & \checkmark & & 0.82 $\pm$ 0.04 & 0.83 $\pm$ 0.05 & 0.81 $\pm$ 0.05 & 0.80 $\pm$ 0.05 \\
                                     & \checkmark & \checkmark & 0.85 $\pm$ 0.03 & 0.85 $\pm$ 0.04 & 0.84 $\pm$ 0.04 & 0.82 $\pm$ 0.04 \\
                                     & & &  0.82 $\pm$ 0.04 & 0.82 $\pm$ 0.05 & 0.81 $\pm$ 0.04 & 0.79 $\pm$ 0.05 \\
        \bottomrule
    \end{tabular}
        \label{tab:ablation_results}
\end{table}


\subsection{Ablation Study}
\label{sec:ablation_study}

Table \ref{tab:ablation_results} presents the results of the ablation study conducted as outlined in Section \ref{sec:exp-procedure}. The second and third columns specify the features present in the training, with the first row for each dataset representing the method in its default configuration.
% , while precision, recall, and F1 Score are reported as macro values.
As observed in the table, the data augmentation had a modest positive impact. The most significant influence on performance was observed for the frames uniformization mechanism, which increased accuracy for LIBRAS-UFOP by 3 percentage points (p.p.). However, it had the opposite effect on MINDS-Libras, resulting in a decrease in accuracy by 5 p.p.

% Given the mixed results from frame normalization, we decided to use the entire video without modifications, as this approach yielded better results compared to other methods for both datasets. This observation suggests that altering frame counts can sometimes enhance accuracy, presenting a valuable area for further investigation.

\subsection{Comparative Evaluation}

% This section delineates the results obtained through our methodology, offers a comparative analysis with contemporary state-of-the-art models applied to both the MINDS-Libras and LIBRAS-UFOP datasets, and discusses the implications of these findings. Initially, a comprehensive table is presented, summarizing the outcomes achieved by all methods. Subsequently, we delve into a detailed exploration of the insights garnered from each dataset. Finally, a critical discussion regarding the proposed method is provided, highlighting its contributions and potential implications for future research in the field.

% All tests on this section were conducted using the LOPO protocol, as described in Experimental Methodology section.

Table \ref{tab:results} provides the results for the comparison with the state-of-the-art on the evaluated datasets. The results of the compared methods correspond to those reported in \cite{DeCastro2023}, and the ``-'' symbol indicates entries for which the metric was not available.
% The results derived from our method are distinguished in bold for ease of identification.
Overall, the proposed method achieved the best performance in all the available metrics. In MINDS-Libras, it outperformed \cite{DeCastro2023} (state-of-the-art) by 2 p.p. in accuracy and 3 p.p. in F1-score, with a lower standard deviation in both metrics. The remarkable point is that our method stands out for its simplicity compared to the complex multimodal 3-D CNN approach proposed in \cite{DeCastro2023}. For the LIBRAS-UFOP dataset, our method outperformed \cite{DeCastro2023} and \cite{Cerna2021} by a larger margin: 8 p.p. in accuracy and 9 p.p. in F1-score.

\begin{table}[t]
    \caption{Results of the comparative evaluation (avg. metric $\pm$ standard deviation). The ``-'' marker indicates that the metric is not available.}
    \label{tab:results}
    \centering
    \begin{tabular}{cccccc}
        \toprule
        Method & Dataset & Accuracy & Precision & Recall & F1-score \\
        \midrule
        \textbf{Ours} & \multirow{3}{*}{MINDS-Libras} & \textbf{0.93  $\pm$ 0.05} & \textbf{0.94 $\pm$ 0.05} & \textbf{0.93 $\pm$ 0.05} & \textbf{0.93 $\pm$ 0.05} \\
        De Castro (2023) \cite{DeCastro2023}  &  & 0.91 $\pm$ 0.07 & - & -          & 0.90 $\pm$ 0.08 \\
        Passos et al. (2021) \cite{Passos2021} &  & 0.85 $\pm$ 0.02 & -             & -          & -             \\
        \midrule
        \textbf{Ours} & \multirow{4}{*}{LIBRAS-UFOP} & \textbf{0.82 $\pm$ 0.04} & \textbf{0.83 $\pm$ 0.05} & \textbf{0.81$\pm$ 0.05} & \textbf{0.80 $\pm$ 0.05} \\
        De Castro (2023) \cite{DeCastro2023} & & 0.74 $\pm$ 0.04 & -             & -          & 0.71 $\pm$ 0.05 \\
        % Cerna et al. (2021) \cite{Cerna2021} & & 0.61 $\pm$ 0.03 & -             & -          & -             \\
        Passos et al. (2021) \cite{Passos2021} & & 0.65 $\pm$ 0.04 & -             & -          & -             \\
        Cerna et al. (2021) \cite{Cerna2021} & & 0.74 $\pm$ 0.03 & -             & -          & -             \\ 
        \bottomrule
    \end{tabular}
\end{table}

% As done in \cite{DeCastro2023}, we also analyze the accuracy across the categories of LIBRAS-UFOP reported in Table \ref{tab:results_ufop_categories}. Our results, highlighted in bold for easy visualization, demonstrate the highest overall accuracy compared to other methods, achieving a value of 0.82. Particularly strong performances were observed in Categories 2 and 4, where we also achieved the highest accuracies reported in the table. While Category 1 showed our lowest accuracy at 0.62, it remains comparable to or better than most of the methods we evaluated.

% \begin{table}[t]
%     \centering
%     \begin{tabular}{cccccl}
%         \toprule
%         Method           & Categ. 1        & Categ. 2        & Categ. 3        & Categ. 4        & All             \\
%         \midrule
%         \textbf{Ours}             & \textbf{0.62 $\pm$ 0.08} & \textbf{0.87 $\pm$ 0.04} & \textbf{0.76 $\pm$ 0.12} & \textbf{0.86 $\pm$ 0.07} & \textbf{0.82 $\pm$ 0.04} \\
%         Cerna et al. \cite{Cerna2021} RGB & 0.62 $\pm$ 0.03 & 0.60 $\pm$ 0.02 & 0.76 $\pm$ 0.01 & 0.60 $\pm$ 0.02 & 0.61 $\pm$ 0.03 \\
%         Passos et al. \cite{Passos2021}    & 0.58 $\pm$ 0.03 & 0.72 $\pm$ 0.01 & 0.93 $\pm$ 0.06 & 0.82 $\pm$ 0.07 & 0.65 $\pm$ 0.04 \\
%         De Castro et al. \cite{DeCastro2023} & 0.60 $\pm$ 0.03 & 0.72 $\pm$ 0.09 & 0.76 $\pm$ 0.07 & 0.83 $\pm$ 0.07 & 0.74 $\pm$ 0.04 \\
%         Cerna et al. \cite{Cerna2021} Kinect & 0.79 $\pm$ 0.04 & 0.72 $\pm$ 0.03 & 0.92 $\pm$ 0.02 & 0.72 $\pm$ 0.02 & 0.74 $\pm$ 0.03 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Results of LIBRAS-UFOP dataset separed by category group.}
%     \label{tab:results_ufop_categories}
% \end{table}

\paragraph{Limitations on Time Efficiency}

% Table \ref{tab:benchmark} presents a comparative view of time performance with respect to the 

A limitation of our approach is the time burden of extracting the landmarks, which in turn is due to the dependency on the OpenPose library. On average, processing a video sequence with OpenPose takes nearly 36 seconds, resulting in an approximate frame rate of 2 frames per second, hindering real-time performance. Nonetheless, the same issue is observed in the method of De Castro et al. \cite{DeCastro2023}. Their 3-D CNN achieves its highest accuracy by utilizing hand and face pose data extracted by OpenPose. Without this data, the accuracy decreases dramatically by more than 25 p.p., as reported by the authors. The rest of our pipeline takes, on average, around 4.58 milliseconds to classify the entire sequence.

% Acho complicado comparar com o De Castro pois usamos plataformas computacionais diferentes}.

% Our CNN model processes 224x224px RGB images, enabling us to train on the entire MINDS-Libras dataset \cite{Rezende2021} in under 39 seconds using the methods outlined in Section \ref{sec:model}. During training, the peak VRAM usage reached 1657MB, while the classification step required only 617MB. This low memory consumption allows the entire pipeline to be efficiently run on a basic GPU.


% Their approach involves selecting the 10 most critical frames for use in the classification process, effectively reducing the data volume and processing time. The classification phase for their model takes 15 milliseconds, culminating in a total processing time of 552 milliseconds per video. Our data preparation step, which involves transforming the landmarks into an image as outlined in Section \ref{sec:image_transformation}, requires less than 1 millisecond. The classification process itself takes 4.58 milliseconds, resulting in a total of approximately 4.58 milliseconds per video.


% benchmark that compares the time invested in landmarks extraction, data preparation, training, and classification stages between the models developed by Guimarães et al. \cite{DeCastro2023} and our own. The training duration mentioned reflects the time taken to train the entire dataset, as outlined in Section \ref{sec:model}, whereas the other values represent the time per video. All durations are measured in milliseconds. Notably, data on landmarks extraction and training duration for Guimarães et al. \cite{DeCastro2023} are not available. The available data indicate that our approach is faster in the stages we could compare.

% \begin{table}[h!]
%     \caption{Performance benchmark comparison for data preparation and classification time, in milliseconds}
%     \label{tab:benchmark}
%     \centering
%     \begin{tabular}{ccccl}
%         \toprule
%         Method & Landmarks Extraction & Data preparation & Training  & Classification \\
%         \bottomrule
%         Guimarães et al. \cite{DeCastro2023} & -                  & 573.59           & -       & 15.2           \\
%         Ours                                                  & 36,367.03            & 0.0001           & 38,827.35 & 4.58    \\
%         \bottomrule
%     \end{tabular}
% \end{table}

% The data preparation steps implemented by Guimarães et al. \cite{DeCastro2023} include background removal, distance and speed inferences, and depth map generation. Their approach involves selecting the 10 most critical frames for use in the classification process, effectively reducing the data volume and processing time. The classification phase for their model takes 15 milliseconds, culminating in a total processing time of 552 milliseconds per video. Our data preparation step, which involves transforming the landmarks into an image as outlined in Section \ref{sec:image_transformation}, requires less than 1 millisecond. The classification process itself takes 4.58 milliseconds, resulting in a total of approximately 4.58 milliseconds per video.

% Our CNN model processes 224x224px RGB images, enabling us to train on the entire MINDS-Libras dataset \cite{Rezende2021} in under 39 seconds using the methods outlined in Section \ref{sec:model}. During training, the peak VRAM usage reached 1657MB, while the classification step required only 617MB. This low memory consumption allows the entire pipeline to be efficiently run on a basic GPU.


% The proposed approach utilizes the entire video frame sequence because we have determined on Section 4.3 that using fewer frames can obscure critical information, thereby negatively impacting model accuracy. This decision directly influences our landmarks extraction process, which takes an average of 36 seconds per video. The majority of this time is spent on extracting landmarks using OpenPose \cite{cao2019openpose}. Although De Castro et al. \cite{DeCastro2023} utilize the same library, their data extraction time has not been disclosed. Future studies could explore methods to reduce the time required for landmark extraction.



